New LP-based Upper Bounds in the Rate-vs.-Distance Problem for Linear Codes

We develop a new family of linear programs, that yield upper bounds on the rate of binary linear codes of a given distance. Our bounds apply {\em only to linear codes.} Delsarte's LP is the weakest member of this family and our LP yields increasingly tighter upper bounds on the rate as its control parameter increases. Numerical experiments show significant improvement compared to Delsarte. These convincing numerical results, and the large variety of tools available for asymptotic analysis, give us hope that our work will lead to new and improved asymptotic upper bounds on the possible rate of linear codes. A concurrent work by Coregliano, Jeronimo, and Jones offers a closely related family of linear programs which converges to the true bound. Here we provide a new proof of convergence for the same LPs.

==> 08_conclusions.tex <==

\section{Conclusions}

\label{section:conclusions}

We introduced a new family of linear programs, $\DelsarteLinCube{r}{n}{d}$,
that yields increasingly tighter upper bounds on the size linear codes. Our LP
family is based on Delsarte's LP and generalizes it. Similar to Delsarte,
symmetrization of $\DelsarteLinCubeNoParams$ yields an exponentially smaller LP
with Krawtchouk polynomials as its main component. Our construction motivated
the definition of the partial Fourier transform.

The big challenge in this area is to improve the asymptotic bounds on the rate
of linear codes. We are inspired by the MRRW bound that,
% does just that with
% Delsarte's LP. This is done 
by finding a good feasible solution to the dual of
Delsarte's LP.
Samorodnitsky et.\ al.\ \cite{samorodnitsky2001optimum,navon2005delsarte}
have explored the limitations
of this approach, 
showing, in particular, that it cannot converge to the
Gilbert-Varshamov bound. 
Barg and Jaffe \cite{barg1999numerical}
argue, based on empirical evidence,
% provided
% empirical evidence suggesting
that
the optimum of Delsarte converges to
the MRRW bound, and therefore it is unlikely that
any improvement will come from
Delsarte's LP.
We believe that our work can lead to such an improvement.

The advantage of $\DelsarteLinCubeNoParams$ over Delsarte's LP
is demonstrated empirically,
already with $r=2$. In the vast majority of the cases
$\DelsarteLinCubeNoParams$ gave substantially better upper bounds than Delsarte.
Notably, in all the instances where
Delsarte's LP does not attain the best known bound for linear codes,
$\DelsarteLinCubeNoParams$ does better. Our numerical results also 
demonstrate the power of the partial Fourier transform, without
which only a modest improvement is attained.

Our numerical experiments do not extend to larger values of $r$
because of high computational complexity already at $r=3$.
One possible way to tackle the computational hardness is by
symmetrizing the LP w.r.t.\ $\GL{r}{2}$. To this end we will need to determine the
orbits of this action, and to compute the symmetrized Krawtchouk polynomials. These
problems may be of independent interest.
 



==> 11_dual_lps.tex <==
\section{Dual Programs and Feasible solutions}\label{section:dual_lps} 

% We choose to formulate the dual of the variation whose objective is
% \eqref{eq:delsarte_lin:objective_span}, and constraints
% \eqref{eq:delsarte_lin:C1}, \eqref{eq:delsarte_lin:C2},
% \eqref{eq:delsarte_lin:C3_span} and \eqref{eq:delsarte_lin:C4}.

We find it conceptually easier to work with the program defined on the cube,
rather than the symmetrized one. The dual can then be symmetrized.

% Let $c:\cube{r\times n} \to \R$ be the coefficients of the objective
% function, i.e.
% \[
%     c(\x) =
%     \begin{cases}
%         (2^r-1)^{-1} & \x=ux^\intercal, 0\neq u\in\cube{r}, x\in\cube{n} \\
%         0 & \text{o/w}
%     \end{cases}
% \]
Let $g_U:\cube{r\times n}\to \R$ be the optimization variables, for $\emptyset
\neq U\subset [r]$. Following is the dual LP, which we denote by
$\DelsarteLinDual{r}{n}{d}$. It is obtained by standard LP manipulations.

\begin{align}
    \underset{\{{g_U:\cube{r\times n}\to\R}\}_{\emptyset\neq U\subset[r]}}
        {\text{minimize}}\quad
    & 1 + \sum_{\emptyset\neq U\subset[r]}\sum_{\x\in\cube{r\times n}}
        \chi^{U}_{\x}(\0) g_U(\x)
    % & 1 + \sum_{\emptyset\neq U\subset[r]}\sum_{\x\in\cube{r\times n}}
    %     \chi^{U}_{\x}(\0) g_U(\x)
    \tag{$d.Obj$}\label{eq:delsarte_lin_dual:objective}
    \\
    \text{subject to}\quad
    & g_U \geq 0 %&& \forall \emptyset\neq U\subset[r]
        \tag{$d.C1$}\label{eq:delsarte_lin_dual:C1}
    \\
    & g_{U}(\mathbf{0}) = 0 %\tag{$C1$}\label{eq:delsarte_lin:C1}
        \tag{$d.C2$}\label{eq:delsarte_lin_dual:C2}
    \\
    & \sum_{T\in GL_r(\cube{})}
        \sum_{\emptyset\neq U\subset[r]} \mathcal{F}_U(g_U)(T\x) \leq 0
        && \text{if } \x \neq \0 \text{ and } \forall u\in \cube{r}:
        \notag
        \\
        &&& |u^\intercal \x|=0
        \vee |u^\intercal \x| \geq d
        \tag{$d.C3$}\label{eq:delsarte_lin_dual:C3}
        % \tag{$C2$}\label{eq:delsarte_lin:C2}
    \\
    & \sum_{0\neq v\in\cube{r}} \sum_{\emptyset\neq U\subset[r]}
        \mathcal{F}_U(g_U)(v x^\intercal)
        \leq -1
        &&  x \in \cube{n}, |x|\geq d
        \tag{$d.C4$}\label{eq:delsarte_lin_dual:C4}
\end{align}

Similarly to the primal, the dual LP is invariant under $\mathfrak{S}_n$ and
$GL_r(\cube{})$.

To see that for for $r=1$ the dual of Delsarte is obtained, note that in that
case the variables are $g\coloneqq g_{[1]}:\cube{n}\to\R$; the constraints
\eqref{eq:delsarte_lin_dual:C3} are implied by \eqref{eq:delsarte_lin_dual:C4},
and thus can be removed; and one can remove the variable $g(0)$ and replace it
with the constant variable $g(0)=1$, while removing the $1$ in the objective
and the $-1$ in the right-hand side of \eqref{eq:delsarte_lin_dual:C4}.

We now show how given a solution to $\DelsarteLinDual{r}{n}{d}$ one can
construct a solution to $\DelsarteLinDual{r+1}{n}{d}$.

Let $g=\{g_U\}_{\emptyset\neq U\subset[r]}$ be a feasible solution to
$\DelsarteLinDual{r}{n}{d}$. We may assume that $g$ satisfies $g(\x)=g(T\x)$
for every $T\in GL_r(\cube{})$, otherwise we can replace it with 
$\overline{g} \coloneqq \frac{1}{|GL_r(\cube{})|} \sum_{T} g(T\x)$.
We shall construct a feasible solution to
$\DelsarteLinDual{r+1}{n}{d}$ with the same value. Let $\mathcal{M}$ be the set
of $r\times(r+1)$ full-rank matrices. Define $g'=\{g'_U:\cube{(r+1)\times n}\to
\R\}_{\emptyset\neq U\subset[r+1]}$ as follows:
\[
    g'_U(\x) =
    \frac{1}{|\mathcal{M}|} \sum_{M\in\mathcal{M}} g_U(M\x)
\]




==> bounds_plot.tex <==
\begin{wrapfigure}{r}{0.35\textwidth}
\begin{center}
\begin{adjustbox}{width=\linewidth}
\begin{tikzpicture}%[font=\tiny]
\begin{axis}[
    grid=major,
    legend pos=north east,
    xlabel={$\delta$},
    ylabel={$\mathcal{R}(\delta)$}
]
    \addplot[ultra thick,color=color4]
        table [x=delta, y=GV, col sep=comma] {data/asymptotic_bounds.csv};
    \addlegendentry{GV \cite{gilbert1952comparison,varshamov1957estimate}}
    \addplot[ultra thick,color=color5]
        table [x=delta, y=MRRW, col sep=comma] {data/asymptotic_bounds.csv};
    \addlegendentry{MRRW \cite{mceliece1977new}}
\end{axis}
\end{tikzpicture}
\end{adjustbox}

\end{center}
\caption{Best known bounds in the
asymptotic rate-vs.-distance.}
\end{wrapfigure}

==> results_plot.tex <==

\begin{figure}[t]
\centering
\makeatletter
\@for\dval:={6,8,10,12,14,16}\do{
\begin{subfigure}[b]{0.3\textwidth}
\centering
\begin{adjustbox}{width=\linewidth}
\begin{tikzpicture}%[font=\tiny]
\begin{axis}[
    % width=1.3\linewidth,
    grid=major,
    legend pos=north west,
    ytick distance=2]
    \addplot[ultra thick,color=color1, mark=o]
        table [x=n, y=delsarte, col sep=comma] {data/plot_table_d_\dval.csv};
    \ifnum \dval=6 {\addlegendentry{Delsarte}} \else {} \fi
    \addplot[ultra thick,color=color3, mark=triangle]
        table [x=n, y=strong_lp, col sep=comma] {data/plot_table_d_\dval.csv};
    \ifnum \dval=6 {\addlegendentry{$\DelsarteLinCube{2}{n}{d}$}} \else {} \fi
    \addplot[thick, dashed,color=black] 
        table [x=n, y=known_bound, col sep=comma] {data/plot_table_d_\dval.csv};
    \ifnum \dval=6 {\addlegendentry{Known bounds}} \else {} \fi
\end{axis}
\end{tikzpicture}
\end{adjustbox}
\caption{$d=\dval$}
\end{subfigure}
}
\makeatother
\caption{
Numerical results comparing 
Delsarte's LP, $\DelsarteLinCubeNoParams$ (our LP with $r=2$),
and the currently best known bounds, as reported in \cite{Grassl:codetables}.
In each plot,
the $x$-axis varies over $n$. The $y$-axis
is the optimal value of the respective linear program,
scaled by $\log_2$.
% is the upper bound obtained from each method,
% % an upper bound 
% on the code's dimension, $\log_2|\C|$,
% where $\C\subset\cube{n}$ is linear with $dist(\C)\geq d$.
Experimental setup, as well as more detailed results,
are given in section \ref{section:numerical_results}.
% obtained from each method.
}
\label{fig:results_plot}
\end{figure}

==> results_plot2.tex <==

\begin{figure}[t]
\centering
\begin{tikzpicture}%[font=\tiny]
\begin{axis}[
    width=\linewidth,
    height=0.5625\linewidth,
    xlabel={$n$},
    ylabel={$\log_2 A(n,d)$},
    grid=major,
    legend pos=north west,
    ytick distance=2
]
\foreach \dval in {6,8,...,16} {
    \addplot[very thick,color=color1, mark=none]
        table [x=n, y=delsarte, col sep=comma] {data/plot_table_d_\dval.csv};
        % \ifnum \dval=6 {node[pos=0,above] {$d=6$}} \else {} \fi
    \ifnum \dval=6 {\addlegendentry{Delsarte}} \else {} \fi
    \addplot[very thick,color=color3, mark=none]
        table [x=n, y=strong_lp, col sep=comma] {data/plot_table_d_\dval.csv};
    \ifnum \dval=6 {\addlegendentry{$\DelsarteLinCube{2}{n}{d}$}} \else {} \fi
    \addplot[dashed,color=black] 
        table [x=n, y=known_bound, col sep=comma] {data/plot_table_d_\dval.csv};
    \ifnum \dval=6 {\addlegendentry{Known bounds}} \else {} \fi
}
\node [anchor=north] at (axis cs:12,4) {\scriptsize $d=6$};
\node [anchor=north] at (axis cs:16,5) {\scriptsize $d=8$};
\node [anchor=north] at (axis cs:20,4) {\scriptsize $d=10$};
\node [anchor=north] at (axis cs:24,5) {\scriptsize $d=12$};
\node [anchor=north] at (axis cs:28,5) {\scriptsize $d=14$};
\node [anchor=north] at (axis cs:32,6) {\scriptsize $d=16$};
\end{axis}
\end{tikzpicture}
\caption{
Numerical results comparing 
Delsarte's LP, $\DelsarteLinCubeNoParams$ (our LP with $r=2$),
and the currently best known bounds, as reported in \cite{Grassl:codetables}.
In each plot,
the $x$-axis varies over $n$. The $y$-axis
is the upper bound obtained from each method,
% an upper bound 
on the code's dimension, $\log_2|\C|$,
where $\C\subset\cube{n}$ is linear with $dist(\C)\geq d$.
Experimental setup, as well as more detailed results,
are given in section \ref{section:numerical_results}.
% obtained from each method.
}
\label{fig:results_plot2}
\end{figure}
